Multi-strange baryon production in pp collisions at $\sqrt{s}$ = 7 TeV with ALICE

A measurement of the multi-strange $\Xi^-$ and $\Omega^-$ baryons and their antiparticles by the ALICE experiment at the CERN Large Hadron Collider (LHC) is presented for inelastic proton-proton collisions at centre of mass energy of 7 TeV. The transverse momentum ($p_{\rm T}$) distributions were studied at mid-rapidity (|y| < 0.5) in the range of 0.6 < $p_{\rm T}$ < 8.5 GeV/$c$ for $\Xi^-$ and $\Xi^+$ baryons, and in the range of 0.8 < $p_{\rm T}$ < 5 GeV/$c$ for $\Omega^-$ and $\Omega^+$. Baryons and antibaryons were measured as separate particles and we find that the baryon to antibaryon ratio of both particle species is consistent with unity over the entire range of the measurement. The statistical precision of the current LHC data has allowed us to measure a difference between the mean $p_{\rm T}$ of $\Xi^-$ ($\Xi^+$) and $\Omega^-$ ($\Omega^+$). Particle yields, mean $p_{\rm T}$, and the spectra in the intermediate $p_{\rm T}$ range are not well described by the PYTHIA Perugia 2011 tune Monte Carlo event generator, which has been tuned to reproduce the early LHC data. The discrepancy is largest for $\Omega^-$ ($\Omega^+$). This PYTHIA tune approaches the $p_{\rm T}$ spectra of $\Xi^-$ and $\Xi^+$ baryons below $p_{\rm T}$ < 0.85 GeV/$c$ and describes the $\Xi^-$ and $\Xi^+$ spectra above $p_{\rm T}$ > 6.0 GeV/$c$. We also illustrate the difference between the experimental data and model by comparing the corresponding ratios of ($\Omega^{-}+\Omega^+)/(\Xi^-+\Xi^+)$ as a function of transverse mass.

==> Makefile <==
all:	default

default:	cds.pdf

cds.pdf:        alice_mspp_cds.dvi alice_mspp_cds.tex
		dvipdf	alice_mspp_cds.dvi alice_mspp_cds.pdf             

alice_mspp_cds.dvi : alice_mspp_cds.tex alice_mspp_cds.bbl
		latex	alice_mspp_cds.tex; \
		latex	alice_mspp_cds.tex; \
		bibtex  alice_mspp_cds; \
		latex	alice_mspp_cds.tex; \
		latex	alice_mspp_cds.tex

alice_mspp_cds.bbl:     alice_mspp_cds.bib
		latex	alice_mspp_cds.tex; \
		latex	alice_mspp_cds.tex; \
		bibtex  alice_mspp_cds


clean-all: clean clean-pdf

clean:	clean-default

clean-pdf:
	rm -rf *.pdf

clean-ps:
	rm -rf *.ps

clean-default: 
	rm -rf *~ *.dvi *.log *.toc *.aux *.tmp *.blg *.out *.spl


# all:	v0.2
# 
# v0.2:	v0.2.ps v0.2.pdf
# 
# v0.2.ps:	alice_mspp_v0.2.dvi alice_mspp_v0.2.tex
# 		dvips	-o alice_mspp_v0.2.ps alice_mspp_v0.2.dvi
# 
# v0.2.pdf:	alice_mspp_v0.2.dvi alice_mspp_v0.2.tex
# 		dvipdf	alice_mspp_v0.2.dvi alice_mspp_v0.2.pdf
# 
# alice_mspp_v0.2.dvi:		alice_mspp_v0.2.tex
# 		latex	alice_mspp_v0.2.tex; \
# 		bibtex  alice_mspp; \
# 		latex	alice_mspp_v0.2.tex;
# 
# clean-all: clean clean-pdf clean-ps
# 
# clean:	clean-v0.2
# 
# clean-pdf:
# 	rm -rf *_v0.2.pdf
# 
# clean-ps:
# 	rm -rf *_v0.2.ps
# 
# clean-v0.2: 
# 	rm -rf *~ *_v0.2.dvi *_v0.2.log *_v0.2.toc *_v0.2.aux *_v0.2.tmp *_v0.2.blg *_v0.2.bbl

